On the generation and propagation of solitary waves in integrable and non-integrable nonlinear lattices

We investigate the generation and propagation of solitary waves in the context of the Hertz chain and Toda lattice, with the aim to highlight the similarities, as well as differences between these systems. We begin by discussing the kinetic and potential energy of a solitary wave in these systems, and show that under certain circumstances the kinetic and potential energy profiles in these systems (i.e., their spatial distribution) look reasonably close to each other. While this and other features, such as the connection between the amplitude and the total energy of the wave bear similarities between the two models, there are also notable differences, such as the width of the wave. We then study the dynamical behavior of these systems in response to an initial velocity impulse. For the Toda lattice, we do so by employing the inverse scattering transform, and we obtain analytically the ratio between the energy of the resulting solitary wave and the energy of the impulse, as a function of the impulse velocity; we then compare the dynamics of the Toda system to that of the Hertz system, for which the corresponding quantities are obtained through numerical simulations. In the latter system, we obtain a universality in the fraction of the energy stored in the resulting solitary traveling wave irrespectively of the size of the impulse. This fraction turns out to only depend on the nonlinear exponent. Finally, we investigate the relation between the velocity of the resulting solitary wave and the velocity of the impulse. In particular, we provide an alternative proof for the numerical scaling rule of Hertz type systems.

==> references3a.tex <==
\catcode`\@ 11
\def\d@mmyjournal{\errmessage{Reference foul up: nested \journal macros}}
\def\@biblabel#1{#1.}

\def\beginblue{\begingroup\color{blue}}
\def\endblue{\endgroup}
	
\begin{thebibliography}{O}

\def\booktitle#1{\textit{#1}}
\itemsep -2pt
\small

%\item[*] Electronic address: biondini@buffalo.edu.~\

% INTRO

\bibitem{kdv}
D. Korteweg and G. de Vries,
\reftitle{On the Change of Form of Long Waves Advancing in a Rectangular Canal, and on a New Type of Long Stationary Waves},
Philosophical Magazine Ser.5, {\bf39}, pp.~422--443 (1895)

\bibitem{Nesterenko}
V.F. Nesterenko,
\booktitle{Dynamics of heterogeneous materials}
(Springer-Verlag, Berlin, 2001)

\bibitem{Nesterenko1}
V.F. Nesterenko,
\reftitle{Propagation of nonlinear compression pulses in granular media},
J. Appl. Mech. Tech. Phys. {\bf24}(5), pp.~733--743 (1983)

\bibitem{sen:2008}
S. Sen, J. Hong, J. Bang, E. $\acute{A}$valos and R. Doney,
\reftitle{Solitary waves in the granular chain},
Phys. Rep. {\bf462}(2), pp.~21-66 (2008)

\bibitem{vakakis} Y. Starosvetsky, K.R. Jayaprakash, M. Arif Hasan,
  A.F. Vakakis,
  \booktitle{Topics on the nonlinear dynamics and acoustics of ordered
    granular media},
  (World Scientific, Singapore, 2017).

\bibitem{chong18} C. Chong, P.G. Kevrekidis,
  \booktitle{Coherent structures in granular crystals},
  (Springer Verlag, Heidelberg, 2018).

\bibitem{IOP}  C. Chong, M.A. Porter, P.G. Kevrekidis, C. Daraio,
  \reftitle{Nonlinear coherent structures in granular crystals},
  J. Phys.: Cond. Matt. {\bf 29}, 413003 (2017).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%\

\bibitem{FrieseckeWattis}
G. Friesecke and J.A.D. Wattis,
\reftitle{Existence theorem for solitary waves on lattices},
Commun. Math. Phys. {\bf161}, pp.~391--418 (1994)

\bibitem{Stefanov}
A. Stefanov and P.~G. Kevrekidis,
\reftitle{On the existence of solitary traveling waves for generalized Hertzian chains},
J. Nonlinear Sci. {\bf22}(3), pp.~327--349 (2012)

\bibitem{Toda}
M. Toda,
\booktitle{Theory of nonlinear lattices}
%Springer series in solid-state sciences~{\bf20}
(Springer-Verlag, 1981)

\bibitem{Toda1}
M. Toda,
\reftitle{Vibration of a chain with nonlinear interaction},
J. Phys. Soc. Jpn. {\bf22}, pp.~431--436 (1967)

\bibitem{Toda2}
M. Toda,
\reftitle{Wave propagation in anharmonic lattices},
J. Phys. Soc. Jpn. {\bf23}, pp.~501--506 (1967)

\bibitem{Toda3}
M. Toda,
\reftitle{Waves in nonlinear lattice},
Prog. Theor. Phys. Suppl. {\bf45}, pp.~174--200 (1970)

\bibitem{Toda4}
M. Toda and M. Wadati,
\reftitle{A soliton and two Solitons in an exponential ;attice and related equations},
J. Phys. Soc. Jpn. {\bf34}, pp.~18--25 (1973)



\bibitem{Hertz}
H. Hertz,
\reftitle{{\"U}ber die ber{\"u}hrung fester elastischer K{\"o}rper} (On the contact of rigid elastic solids),
J. reine und angewandte Mathematik {\bf92}, pp.~156--171 (1881)

\bibitem{Nesterenko2}
V.F. Nesterenko, A.N. Lazaridi and E.B. Sibiryakov,
\reftitle{The decay of soliton at the contact of two `acoustic vacuums'~},
J. Appl. Mech. Tech. Phys. {\bf36}, pp.~166--168 (1995)

\bibitem{Sinkovits}
R. S. Sinkovits and S. Sen,
\reftitle{Nonlinear dynamics in granular columns},
Phys. Rev. Lett. {\bf74}, pp.~2686--2689 (1995)

\bibitem{SenSinkovits}
S. Sen and R.S. Sinkovits,
\reftitle{Sound propagation in impure granular columns},
Phys. Rev. E {\bf54}, pp.~6857--6865 (1996)

\bibitem{Coste}
C. Coste, E. Falcon, and S. Fauve,
\reftitle{Solitary waves in a chain of beads under Hertz contact},
Phys. Rev. E {\bf56}, pp.~6104--6117 (1997)

\bibitem{Hinch}
E.J. Hinch and S. Saint-Jean,
\reftitle{The fragmentation of a line of balls by an impact},
Proc. R. Soc. London, Ser. A {\bf455}, pp.~3201--3220 (1999)

\bibitem{frpego} G. Friesecke, R.L. Pego,
  \reftitle{Solitary waves on FPU lattices: I. Qualitative properties,
    renormalization and continuum limit},
  Nonlinearity {\bf 12}, pp.~1601--1627 (1999).

  % \bibitem{shensen}
\bibitem{Shen}
Y. Shen, P.G. Kevrekidis, S. Sen and A. Hoffman,
\reftitle{Characterizing traveling-wave collisions in granular chains starting from integrable limits: The case of the Korteweg-de Vries equation and the Toda lattice},
Phys. Rev. E {\bf90}(2),~022905 (2014)


\bibitem{pikovsky} K. Ahnert, A. Pikovsky,
  \reftitle{Compactons and chaos in strongly nonlinear lattices},
  Phys. Rev. E {\bf 79}, 026209 (2009).

\bibitem{pegoeng} J.M. English, R.L. Pego,
  \reftitle{On the solitary wave pulse in a chain of beads},
  Proc. Amer. Math. Soc. {\bf 133}, 1763--1768 (2005).

\bibitem{Flashchka1}
H. Flaschka,
\reftitle{The Toda lattice: II. Existence of integrals},
Phys. Rev. B {\bf9}, pp.~1924--1925 (1974)

\bibitem{Flashchka2}
H. Flaschka,
\reftitle{On the Toda lattice: II. Inverse-scattering solution},
Prog. Theor. Phys. {\bf51}, pp.~703--716 (1974)

\bibitem{Henon}
M. Henon,
\reftitle{Integrals of the Toda lattice},
Phys. Rev. B {\bf9}, pp.~1921--1923 (1974)

\bibitem{Venakides}
S. Venakides, P. Deift and R. Oba,
\reftitle{The Toda shock problem},
Commun. Pur. Appl. Math. {\bf44}, pp.~1171--1242 (1991)

\bibitem{Deift}
P. Deift, S. Kamvissis, T. Kriecherbauer and X. Zhou,
\reftitle{The Toda rarefaction problem},
Commun. Pur. Appl. Math. {\bf49}, pp.~35--83 (1996)


\bibitem{NIST}
F W J Olver et al,
\booktitle{NIST Handbook of Mathematical Functions}
(Cambridge University Press, Cambridge, 2010)


\bibitem{cai} D. Cai, A.R. Bishop, N. Gr$\mathrm{\o}$nbech-Jensen,
  Perturbation theories of a discrete, integrable nonlinear
  Schr{\"o}dinger equation,
  Phys. Rev. E {\bf 53}, pp. 4131-4136 (1996). 


\bibitem{SenManciu}
S. Sen and M. Manciu,
\reftitle{Solitary wave dynamics in generalized Hertz chains: An improved solution of the equation of motion},
Phys. Rev. E {\bf64},~056605 (2001)


\bibitem{yuli} Y. Starosvetsky, A.F. Vakakis,
 Traveling waves and localized modes in one-dimensional homogeneous
 granular chains with no precompression,
 Phys. Rev. E {\bf 82}, 026603 (2010).

\bibitem{goldstein}
H. Goldstein, C.P. Poole and J. L. Safko,
\booktitle{Classical mechanics}
(Addison-Wesley, 2001)

\bibitem{sokolow}  A. Sokolow, E. G. Bittle and S. Sen,
  Solitary wave train formation in Hertzian chains,
  EPL {\bf 77}, 24002 (2007).

\bibitem{melo} S. Job, F. Melo, A. Sokolow, S. Sen,
  Solitary wave trains in granular chains: experiments, theory and
  simulations,
  Gran. Matter {\bf 10}, 13-20 (2007).

\bibitem{Panayotis}
P.G. Kevrekidis, A. Vainchtein, M. Serra Garcia, and C. Daraio
Phys. Rev. E {\bf87},~042911 (2013)


%\bibitem{Hoogeboom}
%C. Hoogeboom and P.G. Kevrekidis,
%\reftitle{Breathers in periodic granular chains with multiple band gaps},
%Phys. Rev. E {\bf86},~069903 (2012)

\bibitem{MacKay}
R.S. MacKay,
\reftitle{Solitary waves in a chain of beads under Hertz contact},
Phys. Lett. A {\bf251}, pp.~191--192 (1999)

\bibitem{AS1981}
M. J. Ablowitz and H. Segur,
  \booktitle{Solitons and the inverse scattering transform}
  (SIAM, Philadelphia, 1981)

\bibitem{bloch} A.M. Bloch, Y. Kodama,
  \reftitle{Dispersive regularization of the Whitham equation for the
    Toda lattice},
  SIAM J. Appl. Math. {\bf 52}, pp. 909--928 (1992).

\bibitem{choong}  H. Yasuda, C. Chong, J. Yang, P.G. Kevrekidis
  \reftitle{Emergence of dispersive shocks and rarefaction waves in
    power-law contact models},
  Phys. Rev. E {\bf 95}, 062216 (2017).

  \bibitem{sen:1998}
S. Sen, M. Manciu and J.D. Wright,
\reftitle{Solitonlike pulses in perturbed and driven Hertzian chains and their possible applications in detecting buried impurities},
Phys. Rev. E {\bf57}, pp.~2386--2397 (1998)

\bibitem{Mahan:2008}
S. Neogi and G.D. Mahan,
\reftitle{Generation of traveling solitons in one-dimensional monatomic quartic lattices},
Phys. Rev. B {\bf78},~064306 (2008)


\end{thebibliography}

